pySpatial: Generating 3D Visual Programs for Zero-Shot Spatial Reasoning

Multi-modal Large Language Models (MLLMs) have demonstrated strong capabilities in general-purpose perception and reasoning, but they still struggle with tasks that require spatial understanding of the 3D world. To address this, we introduce pySpatial, a visual programming framework that equips MLLMs with the ability to interface with spatial tools via Python code generation. Given an image sequence and a natural-language query, the model composes function calls to spatial tools including 3D reconstruction, camera-pose recovery, novel-view rendering, etc. These operations convert raw 2D inputs into an explorable 3D scene, enabling MLLMs to reason explicitly over structured spatial representations. Notably, pySpatial requires no gradient-based fine-tuning and operates in a fully zero-shot setting. Experimental evaluations on the challenging MindCube and Omni3D-Bench benchmarks demonstrate that our framework pySpatial consistently surpasses strong MLLM baselines; for instance, it outperforms GPT-4.1-mini by 12.94% on MindCube. Furthermore, we conduct real-world indoor navigation experiments where the robot can successfully traverse complex environments using route plans generated by pySpatial, highlighting the practical effectiveness of our approach.

==> backup.tex <==
% Multi-modal Large Language Models (MLLMs) have achieved remarkable success across diverse general-purpose tasks such as image captioning~\citep{bucciarelli2024personalizing,wu2024visionllm}, referring grounding~\citep{kazemzadeh2014referitgame,mao2016generation}, video understanding~\citep{zeng2025timesuite,fu2025video}, and document parsing~\citep{mathew2021docvqa,mathew2022infographicvqa,luo2024layoutllm}. 
% % Recent efforts have extended these models to higher-level applications like visual navigation and embodied action planning, where language-grounded perception is directly linked to downstream decision-making.

% However, despite their general proficiency, recent studies have demonstrated that current MLLMs face critical challenges in 3D spatial reasoning~\citep{xxx}. These difficulties appear both in simple cases—such as recognizing whether an object is “left,” “right,” “above,” or “below” another in a single image—and in more complex scenarios, such as tracking egocentric motion or reasoning about multi-view relationships across image sequences. The ability to accurately understand and reason about spatial layouts is fundamental for robotics, augmented reality, and embodied AI systems, where tasks like navigation, manipulation, and human–robot interaction rely on precise spatial awareness.


%%% VLM trained on 2D cannot solve,  and VLM trained on 3D (3D alignment) is not very feasible/ scalable
%%% Our approach provide training data for VLM3D

% Recent studies have demonstrated that pre-trained MLLMs perform only slightly above random chance when asked to questions incorporating multi-view spatial reasoning.
% A key limitation lies in the training data: while we have abundant image–text pairs for semantic alignment, explicit 3D supervision is sparse and costly to collect, making large-scale 3D alignment unreliable. As a result, current models often rely on implicit “imagination” mechanisms that fail under realistic settings.

Recent benchmarks highlight this gap. VSI-Bench and MindCube show that pre-trained VLMs perform only slightly above random chance when asked to questions such as, where do I move between two frames.
% A key limitation lies in the training data: while we have abundant image–text pairs for semantic alignment, explicit 3D supervision is sparse and costly to collect, making large-scale 3D alignment unreliable. As a result, current models often rely on implicit “imagination” mechanisms that fail under realistic settings.
% Existing methods largely rely on implicit "imagination" mechanisms, where the model attempts to mentally simulate/speculate spatial layouts or relationships. However, [general VLMs think in 2-D], [training data is rich in semantic labels/image-text alignment but sparse in explicit spatial annotations?], [makes the 3D results unreliable], [limit their use in practical (robotics/auto driving) tasks].
